Electroweak Precision Tests of the Standard Model after the Discovery of the Higgs Boson

The global fit of the Standard Model predictions to electroweak precision data, which has been routinely performed in the past decades by several groups, led to the prediction of the top quark and the Higgs boson masses before their respective discoveries. With the measurement of the Higgs boson mass at the Large Hadron Collider (LHC) in 2012 by the ATLAS and CMS collaborations, the last free parameter of the Standard Model of particle physics has been fixed, and the global electroweak fit can be used to test the full internal consistency of the electroweak sector of the Standard Model and constrain models beyond. In this article, we review the current state-of-the-art theoretical calculations, as well as the precision measurements performed at the LHC, and interpret them within the context of the global electroweak fit. Special focus is drawn in the impact of the Higgs boson mass on the fit.

==> EWFitResultSummary.tex <==
Name
m_{H}
Measurement
125.09
0.15
FitWithoutHiggs
92.0265
33.9789
FitHiggs
92.0265
33.9789
Name
m_{W}
Measurement
80.38
0.013
FitWithoutHiggs
80.3639
0.0170232
FitHiggs
80.3564
0.00613632
Name
#Gamma_{W}
Measurement
2.085
0.042
FitWithoutHiggs
2.09217
0.00145211
FitHiggs
2.09119
0.00126402
Name
m_{t}
Measurement
172.9
0.47
FitWithoutHiggs
177.731
8.04443
FitHiggs
176.45
2.0637
Name
sin^{2}#theta_{eff}(l)
Measurement
0.2314
0.00023
FitWithoutHiggs
0.231393
0.000101803
FitHiggs
0.231514
5.88566e-05
Name
m_{Z}
Measurement
91.1875
0.0021
FitWithoutHiggs
91.1847
0.0239364
FitHiggs
91.2007
0.00927404
Name
#sigma^{0}_{had} 
Measurement
41.54
0.037
FitWithoutHiggs
41.4722
0.0164243
FitHiggs
41.4735
0.0163997
Name
#Gamma_{Z}
Measurement
2.4952
0.0023
FitWithoutHiggs
2.49493
0.00167782
FitHiggs
2.49439
0.00164755
Name
A_{c}
Measurement
0.67
0.027
FitWithoutHiggs
0.668315
0.000322821
FitHiggs
0.667939
0.000200994
Name
A_{b}
Measurement
0.923
0.02
FitWithoutHiggs
0.934703
6.48761e-05
FitHiggs
0.934626
3.85601e-05
Name
A_{l}(SLD)
Measurement
0.1513
0.00207
FitWithoutHiggs
0.147581
0.000787352
FitHiggs
0.146931
0.00046268
Name
A_{l}(LEP)
Measurement
0.1465
0.0033
FitWithoutHiggs
0.147581
0.000787352
FitHiggs
0.146931
0.00046268
Name
A_{FB}^{0,l}
Measurement
0.0171
0.001
FitWithoutHiggs
0.0164051
0.000163065
FitHiggs
0.016227
9.87369e-05
Name
A_{FB}^{0,c}
Measurement
0.0707
0.0035
FitWithoutHiggs
0.0741897
0.00040388
FitHiggs
0.073708
0.000248999
Name
A_{FB}^{0,b}
Measurement
0.0992
0.0016
FitWithoutHiggs
0.104217
0.000560082
FitHiggs
0.103271
0.000323519
Name
R_{l}^{0}
Measurement
20.767
0.025
FitWithoutHiggs
20.7295
0.0271447
FitHiggs
20.723
0.0266492
Name
R_{c}^{0}
Measurement
0.1721
0.003
FitWithoutHiggs
0.172259
8.44933e-05
FitHiggs
0.17225
8.39717e-05
Name
R_{b}^{0}
Measurement
0.21629
0.00066
FitWithoutHiggs
0.215791
0.000112211
FitHiggs
0.215798
0.000112044
Name
#Delta#alpha^{(5)}_{had}
Measurement
0.02758
0.0001
FitWithoutHiggs
0.0281708
0.000912168
FitHiggs
0.0271609
0.000363917
Name
#alpha_{s}(m_{Z})
Measurement
0.1181
0.0011
FitWithoutHiggs
0.119792
0.00295937
FitHiggs
0.119603
0.00295078


==> EWKCommonCommands.tex <==
\newcommand*{\TeV}{\ensuremath{\text{Te\kern -0.1em V}}}
\newcommand*{\GeV}{\ensuremath{\text{Ge\kern -0.1em V}}}
\newcommand*{\MeV}{\ensuremath{\text{Me\kern -0.1em V}}}
\newcommand*{\keV}{\ensuremath{\text{ke\kern -0.1em V}}}
\newcommand*{\eV}{\ensuremath{\text{e\kern -0.1em V}}}
\newcommand*{\ifb}{\mbox{fb$^{-1}$}}
\newcommand*{\ipb}{\mbox{pb$^{-1}$}}
\newcommand*{\inb}{\mbox{nb$^{-1}$}}


==> Table_Theory.tex <==
\begin{table}[tb]
\footnotesize
  \begin{center}
    \begin{tabular}{l | l|l|l|l|l}
\hline
					& Known corrections										& References	& Dominant missing 									&  Theo. unc. 			& Exp. unc. \\
					& 													& 			& orders											&  due to missing orders 	& 		   \\
\hline
$m_W$				& full loop corrections: 									&\cite{Awramik:2003rn}	& $O(\alpha^2\alpha_s), O(\alpha^3)$			& 4 MeV				& 15 MeV	    \\
					& $O(\alpha), O(\alpha_s),O(\alpha\alpha_s), O(\alpha^2)$		&			&												&					&			\\
					& partial loop corrections: 								&			&												&					&		    \\
					& $O(\alpha\alpha_s^2), O(\alpha^2\alpha_s^2m_t^4)$			&			&												&					&			\\
					& $O(\alpha^3m_t^6), O(\alpha\alpha_s^3m_t^2)$				&			&												&					&		    \\
\hline
$\Gamma_W$			& full loop corrections:									&\cite{Kara:2013dua, Denner:1990tx, Alvarez:1987gi,Jegerlehner:1986vs,Bardin:1986fi}			&$O(\alpha\alpha_s), O(\alpha^2), O(\alpha_s^2)$			&					& 42 MeV \\
					& $O(\alpha_s), O(\alpha), O(\alpha \alpha_s)$				&			&												&					&			\\
\hline
$\Gamma_Z$,			&full loop corrections: 									& \cite{Freitas:2014hra, Degrassi:1996ps, Barbieri:1992nz, Freitas:2012sy, Freitas:2013dpa}	& $O(\alpha_{bos}^2), O(\alpha^3)$,		& 0.5 MeV				& 23 MeV\\
$\Gamma_{l\bar l}$,		& $O(\alpha), O(\alpha_s),O(\alpha^2)_{(ferm. loops)}$, 			&			&	$O(\alpha^2\alpha_s), O(\alpha\alpha_s^3)$			& 0.012-0.014 MeV		&		\\
$\Gamma_{q\bar q}$,	& $O(\alpha\alpha_s)$									& 			&												& 0.09-0.21 MeV		&		    \\
$R_l$,				& partial corrections: 									&			&												&$5\cdot10^{-3}$		& $2.5\cdot10^{-2}$	    \\
$R_c$,				& $O(\alpha^2)_{(bos. loops)}$,							&			&												&$5\cdot10^{-5}$		& $3\cdot10^{-3}$	    \\
$R_b$,				& $O(\alpha\alpha_s^3)$,									&			&												&$1.5\cdot10^{-4}$		& $6.6\cdot10^{-4}$	    \\
$\sigma^0_{had}$		&$O(\alpha^2\alpha_s)$, $O(\alpha\alpha_s^2)$				&			&												&					&		    \\
\hline
$\sin^2\theta^l_{eff}$,	& full loops corrections: 									& \cite{Awramik:2008gi, Awramik:2006uz, Dubovyk:2016aqv}		& $O(\alpha^2\alpha_s), O(\alpha^3), O(\alpha\alpha_s^3)$	& $4.4-4.7\times10^{-5}$	&$3.5\cdot10^{-4}$   \\
$A_l$,				& $O(\alpha), O(\alpha_s), O(\alpha\alpha_s), O(\alpha^2)$		&			&												&$3\times10^{-5}$		& $1.8\cdot10^{-3}$ \\
$A_{FB}^{0,f}$,			& partial loop corrections: 								&			&												& $3\times10^{-6}$		& $1.0\cdot10^{-3}$    \\
					& $O(\alpha\alpha_s^2), O(\alpha^2\alpha_s^2m_t^4)$			&			&												&					&			\\
					& $O(\alpha^3m_t^6), O(\alpha\alpha_s^3m_t^2)$				&			&												& 					&		\\
\hline
\end{tabular}
    \caption{Overview of the available oder for the prediction of electroweak precision observables. The missing higher orders as well as their estimated effect on the theory prediction is also given.\label{tab:TheoryOverview}}
  \end{center}
\end{table}

